A geometric characterization of the symplectic Lie algebra

A nonzero element $x$ in a Lie algebra $\mathfrak{g}$ with Lie product $[ , ]$ is called extremal if $[x,[x,y]]$ is a multiple of $x$ for all $y$. In this paper we characterize the (finitary) symplectic Lie algebras as simple Lie algebras generated by their extremal elements satisying the condition that any two noncommuting extremal elements $x,y$ generate an $\mathfrak{sl}_2$ and any third extremal element $z$ commutes with at least one extremal element in this $\mathfrak{sl}_2$.

==> Bibliography8.tex <==

\begin{bibdiv}
\begin{biblist}



\bib{BC13}{book}{
   author={Buekenhout, Francis},
   author={Cohen, Arjeh M.},
   title={Diagram geometry related to classical groups and buildings},
   series={Ergebnisse der Mathematik und ihrer Grenzgebiete. 3. Folge. A
   Series of Modern Surveys in Mathematics [Results in Mathematics and
   Related Areas. 3rd Series. A Series of Modern Surveys in Mathematics]},
   volume={57},
   note={},
   publisher={Springer, Heidelberg},
   date={2013},
   pages={xiv+592},
   isbn={978-3-642-34452-7},
   isbn={978-3-642-34453-4},
   review={\MR{3014979}},
   doi={10.1007/978-3-642-34453-4},
}
\bib{Ben74}{book}{
   author={Benkart, Georgia McClure},
   title={Inner ideals and the structure of Lie algebras},
   note={Thesis (Ph.D.)--Yale University},
   publisher={ProQuest LLC, Ann Arbor, MI},
   date={1974},
   pages={119},
   review={\MR{2625003}},
}


\bib{Ben76}{article}{
   author={Benkart, Georgia},
   title={The Lie inner ideal structure of associative rings},
   journal={J. Algebra},
   volume={43},
   date={1976},
   number={2},
   pages={561--584},
   issn={0021-8693},
   review={\MR{0435149 (55 \#8110)}},
}
\bib{Ben77}{article}{
   author={Benkart, Georgia},
   title={On inner ideals and ad-nilpotent elements of Lie algebras},
   journal={Trans. Amer. Math. Soc.},
   volume={232},
   date={1977},
   pages={61--81},
   issn={0002-9947},
   review={\MR{0466242 (57 \#6122)}},
}
\bib{Blo11}{article}{
   author={Blok, Rieuwert J.},
   title={Highest weight modules and polarized embeddings of shadow spaces},
   journal={J. Algebraic Combin.},
   volume={34},
   date={2011},
   number={1},
   pages={67--113},
   issn={0925-9899},
   review={\MR{2805201 (2012e:20100)}},
   doi={10.1007/s10801-010-0263-3},
}		


\bib{Bou68}{book}{
   author={Bourbaki, N.},
   title={\'El\'ements de math\'ematique. Fasc. XXXIV. Groupes et alg\`ebres
   de Lie. Chapitre IV: Groupes de Coxeter et syst\`emes de Tits. Chapitre
   V: Groupes engendr\'es par des r\'eflexions. Chapitre VI: syst\`emes de
   racines},
   language={French},
   series={Actualit\'es Scientifiques et Industrielles, No. 1337},
   publisher={Hermann, Paris},
   date={1968},
   pages={288 pp. (loose errata)},
   review={\MR{0240238 (39 \#1590)}},
}
\bib{BP03}{article}{
   author={Blok, R. J.},
   author={Pasini, A.},
   title={On absolutely universal embeddings},
   note={Combinatorics 2000 (Gaeta)},
   journal={Discrete Math.},
   volume={267},
   date={2003},
   number={1-3},
   pages={45--62},
   issn={0012-365X},
   review={\MR{1991561 (2004f:51017)}},
}
\bib{BS02}{article}{
   author={Baranov, A. A.},
   author={Strade, H.},
   title={Finitary Lie algebras},
   journal={J. Algebra},
   volume={254},
   date={2002},
   number={1},
   pages={173--211},
   issn={0021-8693},
   review={\MR{1927437 (2003g:17012)}},
   doi={10.1016/S0021-8693(02)00079-0},}
   

\bib{BS74}{article}{
   author={Buekenhout, Francis},
   author={Shult, Ernest},
   title={On the foundations of polar geometry},
   journal={Geometriae Dedicata},
   volume={3},
   date={1974},
   pages={155--170},
   issn={0046-5755},
   review={\MR{0350599 (50 \#3091)}},
}
		


	
\bib{Car72}{book}{
   author={Carter, Roger W.},
   title={Simple groups of Lie type},
   note={Pure and Applied Mathematics, Vol. 28},
   publisher={John Wiley \& Sons, London-New York-Sydney},
   date={1972},
   pages={viii+331},
   review={\MR{0407163 (53 \#10946)}},
}
\bib{CCS99}{article}{
   author={Cohen, A. M.},
   author={Cuypers, H.},
   author={Sterk, H.},
   title={Linear groups generated by reflection tori},
   note={Dedicated to H. S. M. Coxeter on the occasion of his 90th
   birthday},
   journal={Canad. J. Math.},
   volume={51},
   date={1999},
   number={6},
   pages={1149--1174},
   issn={0008-414X},
   review={\MR{1756876 (2001e:20038)}},
   doi={10.4153/CJM-1999-051-7},
}
\bib{Che89}{article}{
   author={Chernousov, V. I.},
   title={The Hasse principle for groups of type $E_8$},
   language={Russian},
   journal={Dokl. Akad. Nauk SSSR},
   volume={306},
   date={1989},
   number={5},
   pages={1059--1063},
   issn={0002-3264},
   translation={
      journal={Soviet Math. Dokl.},
      volume={39},
      date={1989},
      number={3},
      pages={592--596},
      issn={0197-6788},
   },
   review={\MR{1014762 (90m:11055)}},
}
\bib{CI06}{article}{
   author={Cohen, Arjeh M.},
   author={Ivanyos, G{\'a}bor},
   title={Root filtration spaces from Lie algebras and abstract root groups},
   journal={J. Algebra},
   volume={300},
   date={2006},
   number={2},
   pages={433--454},
   issn={0021-8693},
   review={\MR{2228205 (2008a:17008)}},
   doi={10.1016/j.jalgebra.2005.09.043},
}
\bib{CI07}{article}{
   author={Cohen, Arjeh M.},
   author={Ivanyos, G{\'a}bor},
   title={Root shadow spaces},
   journal={European J. Combin.},
   volume={28},
   date={2007},
   number={5},
   pages={1419--1441},
   issn={0195-6698},
   review={\MR{2320071 (2008e:20043)}},
   doi={10.1016/j.ejc.2006.05.016},
}
\bib{CIR08}{article}{
   author={Cohen, Arjeh M.},
   author={Ivanyos, G{\'a}bor},
   author={Roozemond, Dan},
   title={Simple Lie algebras having extremal elements},
   journal={Indag. Math. (N.S.)},
   volume={19},
   date={2008},
   number={2},
   pages={177--188},
   issn={0019-3577},
   review={\MR{2489325 (2010d:17012)}},
   doi={10.1016/S0019-3577(09)00003-2},
}
\bib{CSUW01}{article}{
   author={Cohen, Arjeh M.},
   author={Steinbach, Anja},
   author={Ushirobira, Rosane},
   author={Wales, David},
   title={Lie algebras generated by extremal elements},
   journal={J. Algebra},
   volume={236},
   date={2001},
   number={1},
   pages={122--154},
   issn={0021-8693},
   review={\MR{1808349 (2001k:17007)}},
   doi={10.1006/jabr.2000.8508},
}

\bib{Coh12}{article}{
   author={Cohen, Arjeh M.},
   title={The geometry of extremal elements in a Lie algebra},
   conference={
      title={Buildings, finite geometries and groups},
   },
   book={
      series={Springer Proc. Math.},
      volume={10},
      publisher={Springer, New York},
   },
   date={2012},
   pages={15--35},
   review={\MR{3074860}},
   doi={10.1007/978-1-4614-0709-6-2},
}
\bib{Coh}{book}{
   author={Cohen, Arjeh M.},
   title={Diagram Geometry, Related to Lie algebras and exceptional groups},
   series={ available at www.win.tue.nl/$\sim$amc/buek/book2.pdf},
   volume={},
   note={},
   publisher={preliminary version 2014},
   date={},
   pages={},
   isbn={},
   review={},
}

%\bib{CJP92}{article}{
%   author={Cuypers, Hans},
%   author={Johnson, Peter},
%   author={Pasini, Antonio},
%   title={On the embeddability of polar spaces},
%   journal={Geom. Dedicata},
%   volume={44},
%   date={1992},
%   number={3},
%   pages={349--358},
%   issn={0046-5755},
%   review={\MR{1193124 (94f:51008)}},
%   doi={10.1007/BF00181400},
%}
\bib{CJP93}{article}{
   author={Cuypers, Hans},
   author={Johnson, Peter},
   author={Pasini, Antonio},
   title={On the classification of polar spaces},
   journal={J. Geom.},
   volume={48},
   date={1993},
   number={1-2},
   pages={56--62},
   issn={0047-2468},
   review={\MR{1242702 (94h:51007)}},
   doi={10.1007/BF01226800},
}
		


 \bib{CRS14}{article}{
   author={Cuypers, Hans},
   author={Roberts, Kieran},
   author={Shpectorov, Sergey},
   title={Recovering the Lie algebra from its extremal geometry},
   journal={J. Algebra},
   volume={441},
   date={2015},
   pages={196--215},
   issn={0021-8693},
   review={\MR{3391926}},
   doi={10.1016/j.jalgebra.2015.06.037},
}
\bib{Cuy91}{article}{
   author={Cuypers, Hans},
   title={Symplectic geometries, transvection groups, and modules},
   journal={J. Combin. Theory Ser. A},
   volume={65},
   date={1994},
   number={1},
   pages={39--59},
   issn={0097-3165},
   review={\MR{1255262 (94m:51003)}},
   doi={10.1016/0097-3165(94)90036-1},
}

\bib{CuyFle17}{article}{
  author={Cuypers, Hans},
  author={Fleischmann, Yael},
   title={A geometric characterization of the classical Lie algebras},
   journal={J. of Algebra (to appear)},
   date={2017},
}






\bib{Dip08}{article}{
   author={Draisma, Jan},
   author={in 't panhuis, Jos},
   title={Constructing simply laced Lie algebras from extremal elements},
   journal={Algebra Number Theory},
   volume={2},
   date={2008},
   number={5},
   pages={551--572},
   issn={1937-0652},
   review={\MR{2429453 (2009e:17012)}},
   doi={10.2140/ant.2008.2.551},
}

\bib{Fau73}{article}{
   author={Faulkner, John R.},
   title={On the geometry of inner ideals},
   journal={J. Algebra},
   volume={26},
   date={1973},
   pages={1--9},
   issn={0021-8693},
   review={\MR{0367002 (51 \#3247)}},
}

\bib{Fis71}{article}{
   author={Fischer, Bernd},
   title={Finite groups generated by $3$-transpositions. I},
   journal={Invent. Math.},
   volume={13},
   date={1971},
   pages={232--246},
   issn={0020-9910},
   review={\MR{0294487 (45 \#3557)}},
}

		
\bib{Fl2015}{book}{
   author={Fleischmann, Yael},
   title={A Geometric Approach to Classical Lie Algebras},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2015},
}



\bib{deGr00}{book}{
   author={de Graaf, Willem A.},
   title={Lie algebras: theory and algorithms},
   series={North-Holland Mathematical Library},
   volume={56},
   publisher={North-Holland Publishing Co., Amsterdam},
   date={2000},
   pages={xii+393},
   isbn={0-444-50116-9},
   review={\MR{1743970 (2001j:17011)}},
   doi={10.1016/S0924-6509(00)80040-9},
}

\bib{Hal94}{article}{
   author={Hall, J. I.},
   title={Locally finite simple groups of finitary linear transformations},
   conference={
      title={Finite and locally finite groups},
      address={Istanbul},
      date={1994},
   },
   book={
      series={NATO Adv. Sci. Inst. Ser. C Math. Phys. Sci.},
      volume={471},
      publisher={Kluwer Acad. Publ., Dordrecht},
   },
   date={1995},
   pages={147--188},
   review={\MR{1362809 (96j:20042)}},
   doi={10.1007/978-94-011-0329-96},
}

\bib{Hog82}{article}{
   author={Hogeweij, G. M. D.},
   title={Almost-classical Lie algebras. I, II},
   journal={Nederl. Akad. Wetensch. Indag. Math.},
   volume={44},
   date={1982},
   number={4},
   pages={441--452, 453--460},
   issn={0019-3577},
   review={\MR{683531 (84f:17007)}},
}
\bib{Hum72}{book}{
   author={Humphreys, James E.},
   title={Introduction to Lie algebras and representation theory},
   series={Graduate Texts in Mathematics},
   volume={9},
   note={Second printing, revised},
   publisher={Springer-Verlag, New York-Berlin},
   date={1978},
   pages={xii+171},
   isbn={0-387-90053-5},
   review={\MR{499562 (81b:17007)}},
}
\bib{itp09}{book}{
   author={in 't panhuis, Jos},
   title={ Lie algebras, extremal elements, and geometries},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2009},
}
\bib{itpPR09}{article}{
   author={in 't panhuis, Jos},
   author={Postma, Erik},
   author={Roozemond, Dan},
   title={Extremal presentations for classical Lie algebras},
   journal={J. Algebra},
   volume={322},
   date={2009},
   number={2},
   pages={295--326},
   issn={0021-8693},
   review={\MR{2529091 (2010d:17008)}},
   doi={10.1016/j.jalgebra.2009.04.015},
}
\bib{Jac79}{book}{
   author={Jacobson, Nathan},
   title={Lie algebras},
   note={Republication of the 1962 original},
   publisher={Dover Publications, Inc., New York},
   date={1979},
   pages={ix+331},
   isbn={0-486-63832-4},
   review={\MR{559927 (80k:17001)}},
}
\bib{Joh90}{article}{
   author={Johnson, Peter M.},
   title={Polar spaces of arbitrary rank},
   journal={Geom. Dedicata},
   volume={35},
   date={1990},
   number={1-3},
   pages={229--250},
   issn={0046-5755},
   review={\MR{1066567 (91i:51006)}},
   doi={10.1007/BF00147348},
}
\bib{KS01}{article}{
   author={Kasikova, A.},
   author={Shult, E.},
   title={Absolute embeddings of point-line geometries},
   journal={J. Algebra},
   volume={238},
   date={2001},
   number={1},
   pages={265--291},
   issn={0021-8693},
   review={\MR{1822192 (2003a:51014)}},
   doi={10.1006/jabr.2000.8629},
}

\bib{KS02}{article}{
   author={Kasikova, A.},
   author={Shult, E.},
   title={Point-line characterizations of Lie geometries},
   journal={Advances in Geometry},
   volume={2},
   date={2002},
   number={2},
   pages={147--188},
   issn={},
   review={},
   doi={10.1515/advg.2002.004},
}

\bib{Lef81}{article}{
   author={Lef{\`e}vre-Percsy, C.},
   title={Copolar spaces fully embedded in projective spaces},
   conference={
      title={Combinatorics '81},
      address={Rome},
      date={1981},
   },
   book={
      series={Ann. Discrete Math.},
      volume={18},
      publisher={North-Holland, Amsterdam-New York},
   },
   date={1983},
   pages={553--566},
   review={\MR{695840 (84f:51011)}},
}
		
ISSN 2167-5163
\bib{Pos07}{book}{
   author={Postma, Erik},
   title={From Lie Algebras to Geometry and Back},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2007},
}


\bib{Pre86-1}{article}{
   author={Premet, A. A.},
   title={Inner ideals in modular Lie algebras},
   language={Russian, with English summary},
   journal={Vests\=\i\ Akad. Navuk BSSR Ser. F\=\i z.-Mat. Navuk},
   date={1986},
   number={5},
   pages={11--15, 123},
   issn={0002-3574},
   review={\MR{876665 (88d:17013)}},
}
\bib{Pre86-2}{article}{
   author={Premet, A. A.},
   title={Lie algebras without strong degeneration},
   language={Russian},
   journal={Mat. Sb. (N.S.)},
   volume={129(171)},
   date={1986},
   number={1},
   pages={140--153},
   issn={0368-8666},
   review={\MR{830100 (87g:17018)}},
}		
\bib{Rob12}{book}{
   author={Roberts, Kieran},
   title={Lie Algebras and Incidence Geometry},
   school={PhD thesis, University of Birmingham},
   date={2012},
}

\bib{Ro10}{book}{
   author={Roozemond, Dan},
   title={Algorithms for Lie algebras of algebraic groups},
   school={PhD thesis, Technische Universiteit Eindhoven},
   date={2010},
}
\bib{Ro11}{article}{
   author={Roozemond, Dan},
   title={On Lie algebras generated by few extremal elements},
   journal={J. Algebra},
   volume={348},
   date={2011},
   pages={462--476},
   issn={0021-8693},
   review={\MR{2852252}},
   doi={10.1016/j.jalgebra.2011.10.015},
}
\bib{SvM13}{article}{
   author={Schillewaert, J.},
   author={Van Maldeghem, H.},
   title={Quadric Veronesean caps},
   journal={Bull. Belg. Math. Soc. Simon Stevin},
   volume={20},
   date={2013},
   number={1},
   pages={19--25},
   issn={1370-1444},
   review={\MR{3082740}},
}
\bib{Spr98}{book}{
   author={Springer, T. A.},
   title={Linear algebraic groups},
   series={Progress in Mathematics},
   volume={9},
   edition={2},
   publisher={Birkh\"auser Boston, Inc., Boston, MA},
   date={1998},
   pages={xiv+334},
   isbn={0-8176-4021-5},
   review={\MR{1642713 (99h:20075)}},
   doi={10.1007/978-0-8176-4840-4},
}
\bib{Stb61}{article}{
   author={Steinberg, Robert},
   title={Automorphisms of classical Lie algebras},
   journal={Pacific J. Math.},
   volume={11},
   date={1961},
   pages={1119--1129},
   issn={0030-8730},
   review={\MR{0143845 (26 \#1395)}},
}
\bib{Str04}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. I},
   series={de Gruyter Expositions in Mathematics},
   volume={38},
   note={Structure theory},
   publisher={Walter de Gruyter \& Co., Berlin},
   date={2004},
   pages={viii+540},
   isbn={3-11-014211-2},
   review={\MR{2059133 (2005c:17025)}},
   doi={10.1515/9783110197945},
}
\bib{Str09}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. II},
   series={de Gruyter Expositions in Mathematics},
   volume={42},
   note={Classifying the absolute toral rank two case},
   publisher={Walter de Gruyter \& Co., Berlin},
   date={2009},
   pages={vi+385},
   isbn={978-3-11-019701-3},
   review={\MR{2573283 (2011c:17035)}},
   doi={10.1515/9783110203059},
}
\bib{Str13}{book}{
   author={Strade, Helmut},
   title={Simple Lie algebras over fields of positive characteristic. III},
   series={de Gruyter Expositions in Mathematics},
   volume={57},
   note={Completion of the classification},
   publisher={Walter de Gruyter GmbH \& Co. KG, Berlin},
   date={2013},
   pages={x+239},
   isbn={978-3-11-026298-8},
   isbn={978-3-11-026301-5},
   review={\MR{3025870}},
}
\bib{TVM04}{article}{
   author={Thas, J. A.},
   author={Van Maldeghem, H.},
   title={Full embeddings of the finite dual split Cayley hexagons},
   journal={Combinatorica},
   volume={24},
   date={2004},
   number={4},
   pages={681--698},
   issn={0209-9683},
   review={\MR{2096821 (2005h:51007)}},
   doi={10.1007/s00493-004-0041-8},
}
\bib{Ti74}{book}{
   author={Tits, Jacques},
   title={Buildings of spherical type and finite BN-pairs},
   series={Lecture Notes in Mathematics, Vol. 386},
   publisher={Springer-Verlag, Berlin-New York},
   date={1974},
   pages={x+299},
   review={\MR{0470099 (57 \#9866)}},
}
\bib{Voe89}{article}{
   author={V{\"o}lklein, Helmut},
   title={On the geometry of the adjoint representation of a Chevalley
   group},
   journal={J. Algebra},
   volume={127},
   date={1989},
   number={1},
   pages={139--154},
   issn={0021-8693},
   review={\MR{1029408 (91e:20033b)}},
   doi={10.1016/0021-8693(89)90279-2},
}
\bib{Wei03}{book}{
   author={Weiss, Richard M.},
   title={The structure of spherical buildings},
   publisher={Princeton University Press, Princeton, NJ},
   date={2003},
   pages={xiv+135},
   isbn={0-691-11733-0},
   review={\MR{2034361 (2005b:51027)}},
}
\bib{Wei09}{book}{
   author={Weiss, Richard M.},
   title={The structure of affine buildings},
   series={Annals of Mathematics Studies},
   volume={168},
   publisher={Princeton University Press, Princeton, NJ},
   date={2009},
   pages={xii+368},
   isbn={978-0-691-13881-7},
   review={\MR{2468338 (2009m:51022)}},
}
\end{biblist}
\end{bibdiv}


